Characterizing the MrDeepFakes Sexual Deepfake Marketplace

The prevalence of sexual deepfake material has exploded over the past several years. Attackers create and utilize deepfakes for many reasons: to seek sexual gratification, to harass and humiliate targets, or to exert power over an intimate partner. In part enabling this growth, several markets have emerged to support the buying and selling of sexual deepfake material. In this paper, we systematically characterize the most prominent and mainstream marketplace, MrDeepFakes. We analyze the marketplace economics, the targets of created media, and user discussions of how to create deepfakes, which we use to understand the current state-of-the-art in deepfake creation. Our work uncovers little enforcement of posted rules (e.g., limiting targeting to well-established celebrities), previously undocumented attacker motivations, and unexplored attacker tactics for acquiring resources to create sexual deepfakes.

==> sections/acks.tex <==
% use section* for acknowledgment
\ifCLASSOPTIONcompsoc
  % The Computer Society usually uses the plural form
  \section*{Acknowledgments}
\else
  % regular IEEE prefers the singular form
  \section*{Acknowledgment}
\fi

Bib test~\cite{alkhatib2019street}



==> sections/background.tex <==
\section{Background}

\subsection{Tube Site}

\subsection{Discussion-based Forum}

\subsection{Governance Infrastructure}

\subsubsection{Trust and Reputation}
\myparagraph{Verified Video Creators}{
    To prove you create your own content:
    A creator must provide images of datasets or application, description of their creation process, and a link to ther profile page on \mdf with at least three ``active'' videos (that is, they have not been taken down by moderators). 

    Their account must be at least 30 days old and have e-mail verification, and it must not have any warnings from moderators. 

    Why be verified: earn tokens for video downloads and receive monthly payouts, forum posting privileges in verified creator mega threads, 
}


==> sections/dead/04_vid_results.tex <==
\section{Video}
\label{sec:results}

\subsection{Purpose of videos section}

\subsubsection{Why do people post their videos here?}
\subsubsection{Personal portfolio curation and advertisement} 
Can also go into the video deletion messages here

\subsubsection{Community archive/sharing?}


%%%

\subsection{Targets of \mdf Videos}
\ch{Want to re-think about the terms we use -- target can be conflated possibly to mean the ``body'' due to donor/target terms}
\subsubsection{Gender and sexuality}
\begin{table}[h]
% \small
\centering
\begin{tabularx}{0.9\linewidth}{ X c c }
\toprule
Identity Label         &       \%        &  \# Celebs (of \num{1852})   \\
\midrule          
Woman                  &      95.4       & \num{1767}  \\
Man                    &       2.5       &     46      \\
Transgender            &       0.6       &     12      \\
Nonbinary              &       0.1       &      2      \\
LGBTQIA+               &       2.1       &     39      \\
N/A                    &       1.7       &     31      \\
% Bisexual               &       0.4       &      9      \\
% Pansexual              &       0.1       &      2      \\
% Asexual                &       0.1       &      1      \\
\bottomrule
\end{tabularx}
\vspace{3pt}
\caption{
    Distribution of gender and sexuality categories of celebrities in \mdf videos. 
    Celebrities were assigned multiple labels when appropriate (e.g., a celebrity could be labeled as both ``transgender'' and ``woman'').
    }
\label{tbl:video_celeb_demographics}
\end{table}

Unsurprisingly, the celebrities targeted by sexual deepfake videos on \mdf are almost exclusively women; across our sample of the \num{1852} most frequently targeted celebrities, which accounts for over 99\% of the video subjects, we find that 95.4\% of targeted celebrities are women (Table~\ref{tbl:video_celeb_demographics}). Similarly, we examine the number of videos featuring each gender and sexuality label and find that of the \num{39516} videos that include labeled celebrities, 90.8\% of the videos \textit{solely} depict sexual and gender minorities --- that is, less than 10\% of videos feature any cisgender man. Further, only 186 videos (0.5\%) have cisgender men as their sole subjects.

\ch{Compare to numbers from JOTS and mainstream porn sites, e.g., PornHub, and perform a two-sample proportion test to see if these gender distribtions might be drawn from different populations. Likely they are not for mainstream porn sites.}

\subsubsection{Occupation}
\ch{TODO: the automated part about occupation of high-profile individuals}
Dig into the targeting of niche personas being deepfaked (e.g., OnlyFans creators, local TV news anchors, small cosplayers, retired small actors) --- can point out the ``stalker'' behaviors of some uploaders

Which geopolitical figures are the most popular?

\subsubsection{Nationality}
Dig into the odd exceptions -- South Korean celebrities, from what countries are the geopolitical figures most common or something?

\subsubsection{Desirability?}
What kinds of videos get more engagement, are there any trends here? Or is more based on the user popularity, perhaps?

%%%

\subsection{Norms for deepfake targets}
\subsubsection{Explicit tube rules and guidelines}
\paragraph{\textbf{Upload and content rules}}
    \begin{itemize}
        \item They claim that all videos are moderated
        \item All videos \textit{must} be deepfakes and will otherwise be removed
        \item Only verified creators can monetize their videos and link to external sites
        \item Videos must be at least 30 seconds long --- no slideshows, gifs, video loops
        \item Viewers must be able to \textit{enjoy} your video --- no excessive promotion or obstructive watermarks
        \item Videos must include celebrity name in the title and specify the relevant categories and tags: at minimum, the model ethnicity and ``positions in scenes''
        \item Celebrities must be 18+ years old, follow the guidelines for ``acceptable celebrities'' (~\ref{rules:popularity}), and not be included on the \mdf ``blacklisted'' celebrity list, which handles celebrities that have just turned 18, complicating the legality of the generated content from existing facesets
    \end{itemize}
    
\paragraph{\textbf{Thresholds for popularity on social media}}
\label{rules:popularity}

\paragraph{\textbf{Permissible sexual acts}}

\subsubsection{Distribution of Instagram followers}
Go into the number of videos that violate the explicit rules, maybe an appropriate place to go into the ``verified'' creator process and how they bypass manual review; of the violating videos, how many are posted by verified creators? 

\subsubsection{Violations and Moderation}
\paragraph{\textbf{Verified creators}}

%%%

\subsection{Monetization}
\subsubsection{Cryptocurrency Tipping}

==> sections/dead/05_forum_results.tex <==
\section{Forum}
\label{sec:forum}

\subsection{Market Dynamics}
\subsubsection{Supply and Demand}
Who is being requested --- demographic breakdown?

How much are people charging?

What attributes are creators/sellers advertising (quality, length of video, facesets, iterative feedback)?

%%%

\subsection{Commodity Deepfake Apps}
\subsubsection{Popularity}
\subsubsection{Referral or affiliate-based ecosystem}

%%%

\subsection{Technical Discussion}
\subsubsection{Pain points and constraints}


\subsubsection{Most Cited Research and Open-Source Software}
\paragraph{\textbf{How do these resources navigate or preempt the possible abuse of the technologies?}}

\subsubsection{Comparing hostility or friendliness}
How welcoming is this community compared to more mainstream communities in open-source software or community archives (e.g., Stack Overflow or Wikipedia)?

%%%

\subsection{Ethics and Rules Discussions}
Explicit/implicit for each?
\subsubsection{Permissible Targets}
\subsubsection{Permissible Acts}

%%%

\subsection{Community/Social Network Dynamics}
\subsubsection{Member Reputation}
\subsubsection{Forum Activity}
\subsubsection{Role/Utility of Forum}
\subsubsection{Moderation}
Affirming vs punishing to reinforce norms or rules

==> sections/dead/dead.tex <==
% \todo{start with ``here is what a deepfake is''}
\ch{\textbf{thinking of cutting this text}: In 2017, a Redditor began sharing nonconsensual intimate imagery (NCII) of celebrities' faces swapped onto sex workers' bodies~\cite{cole2017aiassisted}, coining the term ``deepfake'' after their username to refer to media made or manipulated with artificial intelligence (AI) tools.}
% \todo{how the technology has evolved, spectrum of tools}
% In 2019, the \tk company DeepTrace found almost 15K deepfake videos online, of which 96\% were sexual in nature; they report that the ``top four websites dedicated to deepfake pornography'' received over 134M views in aggregate~\cite{}\tk. 
% https://regmedia.co.uk/2019/10/08/deepfake_report.pdf
Advances in deepfake technology have enabled various tools for audio-visual manipulation. These tools balance tradeoffs differently between the required expertise and resources and desired output quality~\cite{paris2019cheapfake}. On one end are commodity ``nudifying'' and ``undressing'' applications that require limited resources and expertise.
% ; reports of the abuse of these apps, especially by middle and high school children to depict their peers, have become increasingly frequent~\cite{tenbarge2024beverly,thorn2023survey}.
On the other end are high-production video-editing software (e.g., that synthesize voices and generate virtual performances) which require deep technical knowledge and resources.
% \todo{reports of its different kinds of abuses}
Many digital threats have operationalized deepfakes, like disinformation campaigns~\cite{dhsincreasing}, financial fraud~\cite{}\tk, and image-based sexual abuse (IBSA)~\cite{hao21horrifying}.
The scale of deepfakes as a form of IBSA has expanded explosively in recent years: female politicians and thousands of celebrities have been targeted~\cite{}, and there are increasing reports of \ch{everyday?} people, including children, depicted in deepfake NCII~\cite{}.
% WSJ: deepfake financial fraud https://www.wsj.com/articles/fraudsters-use-ai-to-mimic-ceos-voice-in-unusual-cybercrime-case-11567157402
% WaPo: deepfakes for scam consumer ads, political ads, nonconsensual sexual imagery: https://www.washingtonpost.com/technology/2024/03/28/ai-women-clone-ads/
% \ch{something about the state of the world: deepfakes have become popularized, commoditized, reports of their abuse by children and of politicians/celebrities}



% \todo{high level overview of prior work in the space of online abuse, then deepfakes more specifically} \todo{what is missing from this body of related work} \ch{while prior work examining mdf exists, the recent surge in public interest in deepfakes is not captured, and its continued growth demonstrates we have not yet figured out how to deal with it}
% \ch{need to massage the intro to this paragraph}
Effectively mitigating online abuse requires solutions for prevention, detection, and triage \ch{harm reduction?}.
While extensive prior work has iterated on improving deepfake detection~\cite{} and finding vulnerabilities in such systems~\cite{} to prevent their amplification, limited research has focused on preventing and triaging~\cite{wei2024understanding} deepfake abuse. 
% Recent work by Wei et~al.\ explores the triaging process for how survivors of IBSA, including those nonconsensually depicted in explicit deepfakes, seek and give help.
Past approaches to preventing online abuse and cybercrime, such as \tk, investigated forum-based communities to inform how attackers \tk. Timmerman et~al.\ study the forum of \mdf, the most prominent ``celebrity deepfake porn tube site,'' to understand the community's attitudes toward the ethics and legality of deepfake creation; however, the economics of the emergent market for sexual deepfakes, as well as how the community identifies and acquires the resources to create deepfakes, remain unexplored. 


A moderator's rule post in the paid requests section warns buyers of fraudulent offers by deepfake creators, suggesting asking for work samples and evaluating the integrity of the account's activity on the forum:
\quoteforum{Keep in mind following - if somoene (sic) is claiming to be able to make you a 20 minute video of some celebrity in less than one day for 50\$ or less - they are probably using single photo swap software you can run yourself, most likely for free and it's not hard to use at all\ldots ask for samples, check their work, do they have other posts or videos on the main site or just "PM me" spam they copy paste into every thread? If the latter be careful too.}


The moderator's warnings suggests that fraudulent offers are common on \mdf, echoing a long history of scams within underground community markets \todo{cite}. We observed three mechanisms buyers use to vet sellers and evaluate their quality and integrity. The primary method is to ask for a portfolio of the seller's past work, as the rule post suggests, and 4.5\% of the requests explicitly asked interested sellers to provide samples; two other requests attempted to evaluate seller quality through first-party trust mechanisms provided by \mdf, such as specifying they wanted a verified seller or a creator with ``great reviews,'' which buyers can leave for verified deepfake video creators in a dedicated thread. 
\ch{is there any grievance airing/bad review mechanism to shame or exile a scammer (like rippers in the past)?}

The rules post also begins to outline the mental model of what factors affect request prices, such as the length of the scene, turnaround time, and video quality. We further document the pipeline for creating a state-of-the-art deepfake video, including the required resources and open challenges, in Section \tk. The rule post also provides concrete guidelines for the market price of deepfake videos so that forum members can operate as informed consumers:

\quoteforum{Ok deepfakes can be had for about 100\$, if you order from well established creator that is known for high quality videos, except to pay anywhere from eve[n] 200-300\$ or more (no upper limit, it's a type of VFX afterall, professional SFW deepfakers can charge upwards of 50\$+ per hour of work... and it takes tens of hours to make high quality deepfake).}

\noindent While no rule requires buyers to publicly advertise a buying price, 11 requests in our sample specified offer prices. We more comprehensively discuss the buyer request prices and seller offer prices across all paid requests threads in Section \tk. 

\begin{table}[h]
% \small
\centering
\begin{tabularx}{\linewidth}{ X X c c }
\toprule
                             &   Attribute         &   \# Requests  &  \% (N=263)  \\
\midrule          
\multirow{2}{=}{Desired Seller Features}   &   Vid. quality   &    32    &  12.0  \\
                            &   Turnaround time   &       5        &  1.9  \\
\addlinespace
\multirow{3}{=}{Seller Vetting}    &   Portfolio         &       12       &  4.5  \\
                             &   Verified status   &       1        &  0.4  \\
                             &   Forum reviews &       1        &  0.4  \\
\bottomrule
\end{tabularx}
\vspace{3pt}
\caption{
    \ch{honestly might kill table and move seller vetting piece to sec 6, keep the seller features here}
    }
\label{tbl:requests_desired_attrs}
\end{table}

\subsection{SOK/Threat Model framing}
\label{ssec:threatmodel}
% \ch{Want to be careful about how we portray the ``sellers'' --- they might not be driving demand themselves, but they are by no means benign or neutral...}
Building upon prior work in the security community~\cite{thomas2021hatesok}, we interpret nonconsensual sexual deepfakes through a threat model that consists of three stakeholders: the \textit{consumer}, the \textit{creator}, and the \textit{target}.\footnote{Drawing upon prior work on online harassment and intimate partner violence, we intentionally use ``target'' over ``victim'' to not disempower those facing abuse.} We define the targets of sexual deepfakes as those whose likeness is abused out of context; however, we recognize that the sex workers whose bodies nonconsensually appear in the videos are also harmed and that characterizing those harms is an area of future work. 

\ch{Not sure if I want to keep this here or move to related work, it kind of breaks the flow in my head but also grounds this ecosystem in a threat model.} Using the taxonomy of online harassment defined by Thomas et al.~\cite{thomas2021hatesok}, we interpret the \textit{audience} of nonconsensual sexual deepfakes as public, given their existence on not only dedicated forums and adult sites, but also on mainstream adult sites\todo{cite?} and social media platforms.\footnote{\todo{Taylor Swift and X, for example.}}
The \textit{medium} of this attack is primarily image and video-based; however, the textual descriptions and titles of these videos often contain the targets' identity and graphic language pertaining to sexual acts. Both the content and the function of the text to optimize discoverability amplify the harm of nonconsensual sexual deepfakes.
While the consumers of deepfakes on \mdf know the media is synthetic, it is unclear to what extent the content is disseminated outside the community and if such attackers must then have the \textit{capability} to deceive a different audience into believing it is real. We further discuss the capabilities required to create deepfakes in Section \TK.


% \chsuggest{figma diagram of buyer/seller/target ecosystem maybe? also brainstorm having two motivation sections, consumer motivation and creator motivation?}


% \todo{better frame this is a marketplace ecosystem to flow into the next paragraph} 

The literature examining image-based sexual abuse (IBSA) has synthesized a list of common perpetrator motives, including sexual pleasure, exertion of power or coercion, circumvention of consent, revenge, proof of masculinity, sextortion, and injury to their target's reputation \todo{cite}. 
% https://vc.bridgew.edu/cgi/viewcontent.cgi?article=3079&context=jiws
Below, we present the underlying motives of the consumers and creators of deepfakes on \mdf; we both situate these actors within existing threat models defined in online abuse literature and identify the differentiating nuances of the deepfake ecosystem.



% The community norms and active participation of \mdf' technically savvy core members have created a hospitable and helpful environment for novice deepfake creators.
Widder et~al.'s study of open source developers of a SFW deepfake creation tool showed that they believed denying technical support for abusive use cases was not only effective, but also their ``best''~\cite{widder2022ethicalai}. However, our exploration of \mdf demonstrates that willing, friendly, and technically capable subcommunities will emerge to address these gaps. 
% \paragraph{Academic and Open Source Contributions}
% \todo{So with that in mind, and the fact that mdf members are arxiv trawlers, shall we more carefully consider the tech we put out into the world with no (or trivial) safeguards?}
Similar to the OSS community, many instances of academic research have used technology neutrality and inevitability to justify the publication and dissemination of innovative developments. We acknowledge that the solution does not lie in silencing research findings or technological innovation, but we argue that ``target hardening'' in the context of mitigating abuse behooves researchers and developers to carefully consider how they choose to distribute their work and preemptively design safeguards to promote intended use/disable or discourage abuse.


\paragraph{Buyer-Target Parasocial Relationships.}
A large body of prior work in psychology has investigated the underpinnings of parasocial interactions and relationships\todo{cite}, and Meloy et al. situate the violent escalation of such parasocial interactions within existing theory for the motivations of stalking public figures. 
The actions of both buyers on \mdf and stalkers of public figures are rooted in the development of a ``narcissistic linking fantasy,'' in which an individual idealizes the object of their fantasy. According to Meloy, the lack of reciprocity between the individual and the object leads to rage, which then becomes the pathway to violence intended to damage or exert control over the object. 
We observe similar sentiments in the request posts, which center on parasocial intimacy with a target and a desire to exert power over them, and believe that situating buyers as subjects of parasocial relationships can inform models for their behavior and thereby ways to discourage their activity. \todo{relate to popova}

\paragraph{Deepfakes as an Art.}
The perception of deepfakes as art and of their consumers as connoisseurs esteems their production with value and purpose. Similarly, the creator of Silk Road, an online black market launched in 2011 that primarily sold drugs, operationalized an ``ideological core'' to give a higher meaning to the online drug trade and moral foundation for community-building~\cite{zajacz2017silk}. An initial study of the \mdf community found that members shared concerns about the suppression of the broader deepfake community following major deplatforming events (from Reddit, Gfycat, Twitter, among others)~\cite{timmerman2023studying}. Together, these attitudes depict a community that perceives itself as a group of creators persecuted for their artistic opinions or sexual preferences, resulting in the community's greater insularity and wariness of outsiders.
% \todo{polarization bit}
% \subsection{Growth of the Deepfake Market}

% \paragraph{Emergent Commodity Ecosystem.}
% \todo{made deepfakes more accessible especially cheapfakes; remind that realism is not where the harm and risk is sometimes, and it appears that cheapfakes are already good enough}
\paragraph{Shifts in the Online ``Fake'' Market}

% The commoditization of deepfake production has significantly lowered the barrier to entry for nonexperts.
A subset of commodity tools has also re-branded deepfake technology as face swapping and ``nudifying'' tools, shedding the negative stigma associated with deepfakes and marketing on mainstream social media platforms to be more palatable for a broader userbase~\cite{maiberg24instagram}.
There have already been several reports of high school children abusing these tools to generate child sexual abuse material by depicting their peers in deepfaked photos~\cite{maiberg24survey,maiberg24instagram,weatherbed2024undressing,koebler24report}, with a recent case where perpetrators locally crowdsourced (e.g., based on school or city) images of non-celebrity, personally acquainted targets and used them generate sexual deepfake images on Telegram~\cite{}\tk.
% ; in fact, based on a 2023 survey from Thorn (a non-profit against child sexual abuse) which reports that one in 10 minors have used ``AI tools to generate nudes of other kids,'' the abuse of deepfake technology is already prevalent~\cite{koebler24report,thorn2023survey}.
We anticipate that increased use of deepfake commodity tools, in ``democratizing'' access to deepfake technology to minors and non-experts, will enable the proliferation of abusive (i.e., child sexual abuse material, nonconsensual) deepfake creation. 
% \todo{cite the bullshit happening in Korean telegram rooms with deepfakes of high schoolers from locally crowdsourced images}

Based on anecdotal evidence on the \mdf forum (Section~\ref{ssec:cost}), commodity deepfake apps and policy criminalizing deepfake NCII appear to have slimmed profit margins. However, this shift may push skilled sellers to offer services for custom content depicting \textit{personal} (rather than ``celebrities'' whose images are publicly available and thereby more easily deepfaked) targets. Further, we expect the maturation of the deepfake market, aligned with economics literature on all labor markets~\cite{}, will lead to a ``deepening'' of skills. Forum discussion indicates that specialization already occurs in a limited capacity (Sections~\ref{subsec:characterization_nonceleb} and~\ref{ssec:cost}), and we anticipate that deepfake creators will increasingly specialize in classes of content or targets to differentiate themselves in a growing labor pool. Our observations suggest that policy solutions may be an effective solution to disincentivize the majority of deepfake creators.

\todo{We need a concluding few sentences of the paper. What does this mean? Where should we go? It just sort of ends right now.}

% \ch{not exactly sure if there's a ``so what'' component here---but I think it's important to predict? idk I think it's cool}

% \paragraph{Deepfake Creator Specialization.}

% \paragraph{Policy Potential.} \ch{aspirational section, not exactly sure what to say/if i am qualified to say anything at all here; however, anecdotally, a mod was complaining about how global outrage/policy enactment criminalizing deepfakes is making monetizing creation harder. while it might push these people to darker/less visible corners of the internet... maybe that's okay. lowkey i predict that this might be where things are headed next, and surviving/dedicated deepfake creators are going to be similar to cybercrime-y people that use a lot of anonymity/privacy preserving technology}




% \subsection{\mdf as a Community}
% \label{ssec:disc_community}
% The norms and values of the \mdf community have created a hospitable environment for inexperienced and curious deepfake creators. \todo{} \ch{talk about how reputation doesn't exactly exist in this ecosystem -- no way to tear down rippers/scammers}

% \paragraph{Deepfakes as an Art.}
% The perception of deepfakes as art and of their consumers as connoisseurs esteems their production with value and purpose. Similarly, the creator of Silk Road, an online black market launched in 2011 that primarily sold drugs, operationalized an ``ideological core'' to give a higher meaning to the online drug trade and moral foundation for community-building~\cite{zajacz2017silk}. An initial study of the \mdf community found that members shared concerns about the suppression of the broader deepfake community following major deplatforming events (from Reddit, Gfycat, Twitter, among others)~\cite{timmerman2023studying}. Together, these attitudes depict a community that perceives itself as a group of creators persecuted for their artistic opinions or sexual preferences, resulting in the community's greater insularity and wariness of outsiders.
% The importance of a shared value system in underground markets predates their emergence online; a 1993 law journal article states that the omnipresence of underground markets indicates that they promote ``widely held societal values''~\cite{priest1993moral}. Applying this to our observations of \mdf points to a set of values concerning NCII held by a growing pocket of society. \ch{something about needing to understand the values and how that affects disincentivizing deepfakes? does such a connection exist? does deplatforming cause more polarization if they perceive themselves as persecuted artists?}

% \subsection{Similarities to Underground Markets}
% \ch{some transition: it's not just the value system that seems familiar between \mdf and predecessor underground markets}
% Past approaches to preventing online abuse and cybercrime, such as \tk, investigated forum-based communities to inform how attackers \tk. Timmerman et~al.\ study the forum of \mdf, the most prominent ``celebrity deepfake porn tube site,'' to understand the community's attitudes toward the ethics and legality of deepfake creation; however, the economics of the emergent market for sexual deepfakes, as well as how the community identifies and acquires the resources to create deepfakes, remain unexplored. 

% \ch{specialization emerging as the market develops -- like we saw with the guatemalan targeting creators}

% \ch{ban of DFL, forks and mirrors available for download elsewhere}

% \subsection{Buyer--Target Parasocial Relationship}

% \noindent A large body of prior work in psychology has investigated the underpinnings of parasocial interactions and relationships\todo{cite}, and Meloy et al. situate the violent escalation of such parasocial interactions within existing theory for the motivations of stalking public figures. 
% The actions of both buyers on \mdf and stalkers of public figures are rooted in the development of a ``narcissistic linking fantasy,'' in which an individual idealizes the object of their fantasy. According to Meloy, the lack of reciprocity between the individual and the object leads to rage, which then becomes the pathway to violence intended to damage or exert control over the object. 
% %https://www.tandfonline.com/doi/pdf/10.1080/00332747.1956.11023049
% %https://www.sciencedirect.com/science/article/pii/B9780124905603500207
% %https://books.google.com/books?hl=en&lr=&id=2ODOTxgmJgEC&oi=fnd&pg=PA287&dq=parasocial+interaction+harassment&ots=aZm65KvKd_&sig=kheZTjIIYdVGsfScS7DDbCrXFio#v=onepage&q=linking%20fantasy&f=false

% We observe similar sentiments in the request posts, which center on parasocial intimacy with a target and a desire to exert power over them. \todo{contrast with the porn studies work.} Related to power and control over targets, prior work in psychology has explored various dimensions of masculinity and its norm scales, including the subordination of women \todo{cite cmni}, dominance, violence, and sexual conquest. We observe expressions of hyper-masculinity in two requests, which situates the range of motives of sexual deepfake buyers within existing models of IBSA perpetrator behaviors --- that is, as motivated by the desire to demonstrate masculinity to a sexually deviant peer network \todo{cite}.


% \subsection{Similarities to Underground Markets}

% \todo{Integrate:} The frequency with which private communication is advertised along with prior analyses of comprehensive logs (i.e., both private and public exchanges) of underground and cybercriminal forums indicate that a large portion of activity --- particularly for the sale and purchase of deepfake content --- likely happen in private channels.
% % Soliciting private or off-platform communication, likely to discuss paid transactions
% The prevalence of ``direct message'' culture in underground forum transactions is often discussed as shady\tk behavior. However, communication research has established that online freelancers also do exactly this; Blyth et al. found that after using a platform to build initial trust with potential clients, freelancers are incentivized to move later exchanges to direct channels to communicate more privately, maintain relationships longitudinally, and make more profit without a middle-man platform~\todo{cite}. Therefore, we argue that understanding similar behaviors in deepfake sellers through the lens of freelancers allows us to model them more as rational economic actors (rather than harm-motivated perpetrators of IBSA) that enable the harms and abuses caused by deepfake consumers. This framing can provide better insight into feasible methods for disrupting this market or disincentivizing its activity.

% \subsection{\mdf as a Community}

% Echoing the model of Silk Road, we argue that the community on \mdf, connected by their perception of deepfakes' artistic value and segregated from mainstream online spaces through deplatforming and stigmatized media narratives \todo{cite}, is a critical component in the establishment and sustained growth of this market. 


% \subsection{Commodity Ecosystem}

% \subsection{Academic and Open Source Contributions}







% % \ch{I really like the idea of connecting evidence of deepfake creators' financial motivation to introduce a new lens with which to understand their psyche: some might indeed be more aligned with the classical model of IBSA (e.g., seeking sexual gratification, revenge), but others are more akin to online freelancers. This wider-spectrum framing allows us to better understand the ecosystem, and while this might not be shocking once you think about it, this allows us to understand their behaviors better (and thereby facilitate disincentivizing such activity). It also dissuades the research community from perceiving patterns of behavior of synthetic IBSA perpetrators as beyond comprehension or specific to members of underground communities --- ``demystifies'' them, if you will.}
% % Digital freelancing related work:
%     % On portfolios, building a brand, connecting to a relevant community in an online, performative way (like being active in MDF) [1, 3]
%     % Building and maintaining these social relationships over time to bolster their platform reputation [1, 2, 3]
%     % Affordances of MDF that reward activity for creators (e.g., designated places to link to your MDF video profile/portfolio, chronological sort of MDF videos by default) [1]
%     % Above relates also to digital freelancer portfolios being reimagined as "temporally dynamic" -- constantly updated, feed-based [1]
%     % Move to off-platform communication among freelancers motivated by: increasing privacy, maintaining relationships, and gaining money, where platforms are crucial in building the initial trust [2]
    
% % [1] https://journals.sagepub.com/doi/full/10.1177/1461444819833066
% % [2] https://journals.sagepub.com/doi/full/10.1177/14614448221108960
% % [3] https://journals.sagepub.com/doi/full/10.1177/1470593115607942
